Deep Model Merging: The Sister of Neural Network Interpretability -- A Survey

We survey the model merging literature through the lens of loss landscape geometry to connect observations from empirical studies on model merging and loss landscape analysis to phenomena that govern neural network training and the emergence of their inner representations. We distill repeated empirical observations from the literature in these fields into descriptions of four major characteristics of loss landscape geometry: mode convexity, determinism, directedness, and connectivity. We argue that insights into the structure of learned representations from model merging have applications to model interpretability and robustness, subsequently we propose promising new research directions at the intersection of these fields.

==> sections/_outline.tex <==

\clearpage


\section{Ideas}

\begin{enumerate}
    \item train models on disjoint data subsets \\
    I would say lets start with two disjoint datasets and then add leakage of data (e.g., set$_1 = \{ 100\% A, 100\% B, x\% C, x\% D \}$ while set$_2 = \{ x\% A, x\% B, 100\% C, 100\% D  \}$)
    \item writing custom transformer modules
    \item recreate subsets paper for transformers
    \item Two ``endpoint'' models initialized to a model trained on two different sets of data
    \item Single model trained end to end: will outperform merged model
    \item Merged model might outperform Single model pipleine based on initial GitRe Basin
    \item Action item: small proof of concept with ResNet Imagenet (merge models trained on disjoint subsets), do this same experiment with transformers (learned subspace (re-implementation), optimize for the lambdas for model merging (our contributions))
    \item Action item \#2: Figure out what to do next
    \item Literature review: Mansi
\end{enumerate}


For the attention layer, we had different ideas
\begin{enumerate}
    \item Just merge them without any logic
    \item Identify similar regions and merge those
    \item Daniel proposed to keep Q and V fixed (?) and just train the other other values
    \item How about merging the layers beforehand from the models to create a 'virtual' layer and train the attention completely on this 'virtual' layer from scratch instead of trying to merge the attention layer?
\end{enumerate}






\section{Introduction}
\label{sec:introduction}
% \input{sections/intro}
[Applicability of model merging to safe and trustworthy ML]

contributions:
\begin{enumerate}
    \item we present a taxonomy of model merging techniques
    \item we explicitly explore the relation between merging learned representations and the underlying nature of the loss landscape
    \item by analyzing various techniques' shortcomings and assumptions we draw meaningful, testable conclusions about the nature of model representations and when they are amenable to being compared 
    \item we draw on our literature survey to provide an in-depth analysis into how fundamental units of model analysis such as architecture, width, and depth intertwine to produce representations of a particular nature
    \item we use information from the model merging literature to directly propose promising directions of research for model interpretability in relation to safety and trustworthiness
\end{enumerate}


\section{Background}

\section{Related Work}
% \include{sections/related_works}

\subsection{The Ensembling Paradox}
The goal of merging models. Ensembling as an upper bound. Multitask learning as an upper bound.

Why, when we have sufficient capacity can we not combine two models to get superior performance to MTL? (Probably because of the data they're trained on).

In practice task representations are compressed to a significantly smaller subspace (even <1\% of the model size) - this further complicates the question of why merging techniques can't approach ensembling accuracy. (Aghajanyan 2020)

If ensembling works, why is merging so lacking?


\subsection{Weight Averaging}
Discussion of all the schemes that are more or less directly averaging weights with some algorithm, without regard for architectural constraints (perm. symmetries).

Touch on the fact that for ALL of the below methods, this only works well when we share a significant portion of the training trajectory (i.e. we have two fine-tuned models from the same pretrained checkpoint as in modern LLM deployments), i.e. weight averaging works when models are already close in space



\subsubsection{Simple Averaging}
May be successful because it interpolates features  (Zhou '24 CTL), which explains the simple success of things like RegMean as well. But why does interpolating features correspond to any improvement in performance?

\subsubsection{Task Arithmetic}
The success of this method points to the similarity in representations learned by models with similar trajectories, especially the transferability between learned features. (This also has a connection to the thesis behind meta-learning, that task-specific parameters will be close to a pre-trained meta-learner see: MAML).

In fact, LoRA operates on this assumption in order to quickly switch out fine-tuning weights for inference

Also, the success of the evolutionary merging approach using task arithmetic/TIES/DARE from Akiba '24 shows that models from the same foundation model can learn transferable features in finetuning.

\subsubsection{Fisher Averaging}
original + MATS approach to approximating more of the fischer matrix

These approaches attempt to estimate the fischer info for each parameter and use it as a weighting for its importance in the final interpolated model. Require a full forward and backward pass over some examples to compute this. The full matrix is far too large, so these approximate the diagonal or get a block-diagonal approximation (MATS)

\subsubsection{RegMean}
Interpolates between model activations to produce the intended result. Is extremely competitive and is even within a percentage point of the MATS approach, while only requiring a single forward pass over a set of examples.

Importantly, permutation-based methods align neurons but keep their activations the same - so regmean actually circumvents the permutation alignment problem because it is only concerned with interpolating between activations - which are already layerwise permutation invariant

This method only checks this for models from the same pretrained checkpoint, but it would be interesting to see if this is successful in other scenarios as well


\subsection{Loss Landscapes and Mode Connectivity}

Concepts to touch on - 
\begin{enumerate}
    \item Mode Determinism - modes are determined very early in training trajectory
    \item Mode Connectivity - permutation symmetries connect equivalent modes 
    \item Mode Convexity - modes are locally convex, admitting interpolation between models in a given mode
    \item Mode Directedness - directions in parameter space correspond to semantic behaviors associated with tasks in a hierarchical fashion (all NLP tasks are clustered, within those are regions where subtask modes lie, and within those are regions corresponding to optimal solutions from a given data distribution).
\end{enumerate}

The principles of mode connectivity are the underpinning for permutation-based approaches. The single loss-basin hypothesis is something that is explored by papers like git-rebasin.

Gueta '23 -> merging models in the same region gives enhanced performance on both the original fine-tuning task and on general tasks in that domain.

Wortsman '21 -> we can find regions of the loss landscape where models are mode-connected by jointly tuning the endpoints of a simplex where interpolating within the region improves task performance even comparable to ensembling accuracy when done in a layerwise fashion.

Yamada '23 suggest that permutation-based methods do not actually reduce L2 distance between models but that they are principally successful because they align singular vectors without changing the singular values and hence "retain similar functionality", making it easier to find mode connected regions. In general they find that independently trained models have very similar singular values, lending some credence to the idea that permuting the singular directions may align the intended functionality of neurons from different models. This is also reflected by Simsek's conclusion that permutation equivalent basins dominate the landscape in overparameterized models.

Modes (connected modes) have semantic importance with respect to model behaviors and properties, Tatro 2020 showed that adversarially robust models when permutation-aligned could be interpolated to find more accurate but still robust models.

\subsection{Permutation Based Methods}

\subsection{Git:Rebasin}
\subsection{Optimal Transport Fusion}
Git rebasin finds a subset of the solutions that otfusion finds. OTfusion finds any transport map, including permutation matrices whereas git rebasin only performs combinatorial optimization over the set of permutation matrices for each layer. I.e. the linear program both of these papers solve exists on the Birkhoff polytope, the solutions to such a program are at the extrema, which correspond to the set of permutation matrices in the case of the set of bistochastic matrices. OT Fusion finds some benefit from having additional "soft" solutions available

OT fusion does only one pass over the layers, greedily aligning them in contrast to git rebasin which repeatedly iterates over all layers until no further benefit is derived in terms of alignment. Despite this, both methods complete in a matter of seconds - though notably git rebasin is written in JAX as opposed to OTFusion's pytorch impl, so comparisons on runtime are hard to make as the underlying code optimization is different.

OTFusion also has a follow-up that does this for transformers whereas gitrebasin doesn't have an implementation that handles this.

Neuron Alignment (Tatro 2020) also explores permutation alignment in a framework similar to that of OTfusion with a cost function based on the correlation between the activations of two neurons.

Zhou '23 (LLFC) provides justification for why such methods might work in theory.

\subsection{Merging with Different Data Distributions}
Both the above try to do this, but aren't super successful (show some promise)

Yamada '23 show a good way to do this using the STE method from rebasin and dataset condensation from Zhao '21.

Yamada '24 suggests that STE uses loss geometry whereas WM exploits linear algebraic properties of the weight matrices.

\section{The effect of architecture on model representations}

\subsection{architecture}
This is explored really well in regmean and MATS, which test various architectures and show the effect of various merging techniques as they vary by base architecture. though all use fine-tuned models from pre trained checkpoints.

\subsection{width and depth}
Some exploration of this is covered in git-rebasin but mostly prospectively. Perhaps some experiments would be useful for this section (we have some code that does this already, just have to extend it to more methods/architectures)

simsek'21 presents a good theoretical analysis of loss landscapes under wider (and to some degree, deeper) neural networks. In particular they state that the loss landscapes of vastly overparameterized neural networks are dominated by connected subspaces of global minimizers (in relation to the number of permutation-symmetry induced saddle points). This suggests that overparameterized networks experience more amicable loss landscapes compared to their underparameterized counterparts. Additionally this could also explain git rebasins observation that wider networks perform better under weight matching - there are simply more equivalent solutions in existence.

\section {The effect of training trajectory on the similarity of learned representations}
an analysis covering task arithmetic, weight averaging schemes, and how permutation-based methods can align certain models - and crucially how permutation-based methods are not necessarily applicable when models share a trajectory (see appendix of regmean).

some works use a gradient regularization to bias solutions toward wide loss basins with small gradient norms and show better generalization properties with this approach, would this also affect the ability to find permutation symmetries/weight average?

ito '24 $\rightarrow$ : (i) the proportion of dominant singular values decreases as
the model width increases, and (ii) the WM preferentially aligns the directions of singular vectors corresponding to such
dominant singular values. (Experiments showing whether RegMean has any consistently noticeable effects on singular vectors would be interesting) 

Zhou '24 CTL - feature linearity within modes

Some visualizations of where models land in space would be good too.

\subsection{real-life deployments}
Does this mean that production deployments of LLMs using openly available pre-trained checkpoints are more vulnerable to attacks? (Because experimenting on pre-trained checkpoints could give non-trivial information with regards to the underlying learned representations)


\section{When does it make sense to compare representations?}

\subsection{Merging between different datasets}
this is more difficult, because of our concerns about training trajectory/loss landscape/optima? because of coordinate permutations/misalignment? because of feature dissimilarity?

Yamada '23 $\rightarrow$ Adding dataset info increases performance in the different-distribution case, can use dataset condensation to reduce cost of this procedure. Their work shows that when dealing with different loss landscapes it is very helpful for performance to have loss information from the datasets available to navigate to regions with low loss barriers

This seems to suggest that STE is more generally applicable than weight matching. Yamada '24 proposes the idea that permutations principally act to align singular directions of models before merging which makes finding mode-connected regions easier. The fact that STE is more useful for different data distributions probably reflects the fact that both singular directions and values are misaligned with respect to functionality. Whether this holds true is an open question that has not been investigated as of yet (!!!). This also might have implications for task transfer between related and disjoint tasks, picking a few directions with high singular values and "fitting" them so to speak inside of a model by choosing the singular directions carefully could be a promising direction of research, but has not been tried yet (!!!). This idea is similar to the idea of continual learning in orthogonal subspaces.

What does the distribution of singular values look like when we do multi-task learning on diff. datasets vs training models on disjoint subsets of a dataset (OPEN QUESTION !!!)? Can we merge these models by fitting their singular vectors into orthogonal subspaces?

If two models achieve low loss, then their likelihood under the corresponding Gibbs distribution for that loss function is high (i.e. SGD will likely converge to one of these states, over an arbitrary state). When we consider two models trained on disjoint subsets of a given dataset (effectively two different datasets), then their loss is high wrt the full dataset, making them unlikely under the corresponding gibbs distribution - can we characterize merging failures using this perspective? Ito '24 use STE for merging between two diff datasets by minimizing $L_{ab}$ with $params_b^*$. However their solutions find endpoints with high loss, though the region between the two endpoints does better than the two endpoints (by 30 points in accuracy).

What is the relationship between the loss landscapes of a task and a sub-task? What is the relationship between loss landscapes of two different problems in the same domain?

\section{Open questions/Interpretability research directions}
Entropy-SGD seeks to find wider minima - can their logic be applied to using STE for merging from different datasets?

Opportunity: existing methods all take the perspective that models should be merged in parameter space, but can we benefit more from an alternative perspective? Namely that we are interpolating functions and should focus on viewing neural networks as a series of linear maps interspersed with non-linearities as RegMean does? Focusing instead on the actual nature of the linear transformations we have learned during training promises to allow greater reuse of theoretical machinery that has already been studied in linear algebra and functional analysis and offers the opportunity to develop algorithms with provable guarantees as far as the correctness of the final merged model.

The success of layerwise merging techniques in approaching ensembling accuracy (wortsman '21) implies that the above approach is reasonable and perhaps more performant and this makes sense from a theoretical point of view.

Do works like Zhou '24, cross-task-linearity, show promise for this and a theoretical direction? Focusing on feature space could be a good investment.


Continuous learning in orthogonal subspaces, stuffing models into orthogonal subspaces?

Bin-packing models into an architecture with extreme pruning or parameterization techniques like SAID (Aghajanyan 2020)

Do these works suggest that NN architectures could benefit from reparameterizations that differ from the current standard MLP architecture but are equally universal?

\section{Future Works (``Hot Takes'')}
...

Actually, naive interpolation of matrices will produce skew and volume deformations that are not intended - in reality we should perhaps decompose each matrix into a rotation, scaling, and translation and then individually interpolate each of those - crucially, they must each be treated differently. For example while scaling and translation along each dimension could be linearly interpolated, rotations must be spherically interpolated. In theory we should actually consider the transformation from the entire network - however, empirical evidence suggests that it is reasonable to do this procedure layerwise.

==> sections/conclusion.tex <==
...

==> sections/data_aware_table.tex <==
\begin{longtable}{|P{0.15\textwidth}|P{0.34\textwidth}|P{0.09\textwidth}|p{0.4\textwidth}|}
\hline
Classification & Name & Source & Summary \\
\hline
Data-Aware
  & FedAvg
  & \citet{sun2022decentralized} 
  & Computes a weighted average between source model parameters in a federated setting. Weights each source model's parameters by the proportion of the data in the federated system that is present at their node. Suitable for merging models whose data distributions are heterogeneous and non-IID. \\
\cline{2-4}
  & AdaMerging
  & \citet{yang2023adamerging} 
  & Builds upon Task Arithmetic~\cite{ilharco2022editing}. Learns merging coefficients for task vectors adaptively by minimizing prediction entropy over unlabeled test data. Demonstrates strong multi-task performance, comparable with that of an ensemble. \\
\cline{2-4}
  & RegMean
  & \citet{jin2022dataless} 
  & Merges weights at each layer by computing the least-squares fit to their activation maps. This ensures that the merged weight matrix produces activations similar to that of each source matrix when presented with data from that source model's training distribution.  \\
\cline{2-4}
  & ZipIt!
  & \citet{stoica2023zipit} 
  & Identifies redundant parameters between models whose activations are highly correlated. This technique only merges redundant model parameters and preserves task-specific ones to prevent destructive interference when merging models. Demonstrates strong multi-task performance, even when models are trained independently.  \\
\hline
\end{longtable}

==> sections/experiments.tex <==
...

==> sections/hard_alignment_table.tex <==
\begin{longtable}{|P{0.15\textwidth}|P{0.34\textwidth}|P{0.09\textwidth}|p{0.4\textwidth}|}
\hline
Classification & Name & Source & Summary \\
\hline
Hard Alignment
  & Weight Matching 
  & \citet{ainsworth2022git}
  & Aligns corresponding layers of neurons between models of the same architecture by maximizing the similarity between their weight matrices (i.e., maximizing the Frobenius inner product of both weight matrices). They pose this problem as an NP-hard SOBLAP assignment problem and approximate a greedy solution using coordinate descent. Once weights are aligned, they are simply averaged. \\
\cline{2-4}
  & Optimizing Mode Connectivity via Neuron Alignment
  & \citet{tatro2020optimizing} 
  & Presents a heuristic, \enquote{neuron alignment}, which measures similarity between the distribution of activations between two weight matrices. They relate finding a permutation matrix which optimizes this metric to the assignment problem~\cite{burkard1999linear} and optimal transport. Weights are interpolated between once aligned.  \\
\cline{2-4}
  & Probabilistic Federated Neural Matching (PFNM)
  & \citet{yurochkin2019bayesian} 
  & Aligns the parameters of edge models to a global model in a federated setting by using a non-parametric Bayesian model to determine the optimal assignment of neurons to one another for alignment and merging into a global model.  \\
\cline{2-4}
  & Federated Learning with Matched Averaging (FedMA)
  & \citet{wang2020federated} 
  & Poses neuron alignment as an extended bipartite matching problem and applies the iterative Hungarian matching algorithm to solve the corresponding assignment problem, aligning neurons before merging.  \\
\hline
\end{longtable}

==> sections/info_theoretic_table.tex <==
\begin{longtable}{|P{0.15\textwidth}|P{0.34\textwidth}|P{0.09\textwidth}|p{0.4\textwidth}|}
\hline
Classification & Name & Source & Summary \\
\hline
Information Theoretic
  & Fisher Weighted Averaging
  & \citet{matena2022merging} 
  & Computes a weighted average between source model parameters, with weights for each parameter defined by the Fisher information of that parameter. Applies a diagonal approximation of the Fisher Information matrix for computational tractability. \\
\cline{2-4}
  & Merging by Matching Models in Task Parameter Subspaces (MaTS)
  & \citet{tam2023merging} 
  & Poses model merging as equivalent to solving a linear system of equations for the optimal merged parameter values. They design an enhanced Fisher Weighted Averaging procedure by using the Kronecker Factorization to obtain a more accurate block-diagonal approximation to the Fisher Information matrix. Computing the closed-form solution to this system is intractable in practice; therefore, they apply the method of Conjugate Gradients to find an approximate solution.  \\
\hline
\end{longtable}

==> sections/new_survey_table.tex <==
\begin{table}[ht]
\label{tab:taxonomy}
\caption{Table of Model Merging techniques covered in this work, categorized by their approach.}

\footnotesize
\begin{adjustbox}{max width=\textwidth, angle=0}
% \begin{tabularx}{\textheight}{p{0.15\textwidth}p{0.15\textwidth}p{0.2\textwidth}p{0.2\textwidth}p{0.5\textwidth}}

\begin{tabular}{
    p{0.1\textwidth}
    p{0.1\textwidth}
    p{0.15\textwidth}
    p{0.15\textwidth}
    p{0.7\textwidth}
}
\toprule
    Classification & Type & Name & Source & Summary \\
\midrule
\multirow{16}{\subwidth}{Ensembling}
  & \multirow{9}{\subwidth}{Predictive} 
  & Snapshot Ensembles
  & \citet{huang2017snapshot}
  & Cycles through learning rates during training to obtain several models in distinct minima, averages their logits during inference. \\
\cmidrule{3-5}
  &
  & Fast Geometric Ensembling
  & \citet{garipov2018loss}
  & Trains a single neural network traditionally for approximately 80\% of the time until convergence, then employs a dynamic learning rate schedule to obtain several models with low loss to eventually ensemble their logits. \\
\cmidrule{3-5}
  &
  & Simplices for Fast Ensembling
  & \citet{benton2021loss}
  & Trains several models to find a trivial simplicial complex of low loss solutions, then trains several \enquote{connecting} solutions such that we are left with a full simplex of low loss solutions for ensembling. \\
\cmidrule{2-5}
  & \multirow{6}{\subwidth}{Compositional}
  & Mixture-of-Experts (MoE)
  & \citet{shazeer2017outrageously}
  & MoE maintains a cohort of \enquote{experts}---specialized subnetworks of neurons---and learns a routing network which then selects the top-$k$ experts for any given input and outputs a linear combination of each of their predictions. \\
\cmidrule{3-5}
  &
  & Switch Transformers
  & \citet{fedus2022switch}
  &  Simplifies the MoE router by demonstrating that just a single expert per input example is sufficient for strong performance. Significantly reduces communication and computational costs enabling superior scaling of MoE models. \\
\midrule
\multirow{57}{\subwidth}{Weight Aggregation}
  & \multirow{14}{\subwidth}{Weight Averaging} 
  & FedSGD (Simple Average)
  & \citet{mcmahan2017communication} 
  & Computes a simple average over source model parameters. Requires models of the same architecture. \\
\cmidrule{3-5}
  & 
  & Stochastic Weighted Averaging 
  & \citet{izmailov2018averaging} 
  & Gathers checkpoints from various points in the training trajectory of a single model and computes a simple average over their parameters. \\
\cmidrule{3-5}
  & 
  & \multirow{2}{\subwidth}{Model Soup}
  & \citet{wortsman2022model} 
  & Takes the simple average of parameters from models of the same architecture fine-tuned with different hyperparameters. \\
\cmidrule{3-5}
  & 
  & Sparse Soup 
  & \citet{zimmer2023sparse} 
  & Constructs model soups that are more efficient for inference by applying a technique inspired by Iterative Magnitude Pruning~\cite{tanaka2020pruning} to produce sparse models. \\
\cmidrule{3-5}
  & 
  & SWAMP 
  & \citet{choi2023swamp} 
  & Iteratively applies Iterative Magnitude Pruning~\cite{tanaka2020pruning} and simple weight averaging between multiple fine-tuned models to produce a final sparse, merged model. \\
\cmidrule{2-5}
& \multirow{17}{\subwidth}{Weight Steering} 
  & \multirow{4}{\subwidth}{Task Arithmetic}
  & \citet{ilharco2022editing} 
  & Computes a \enquote{task vector}: the difference between the pre-trained and fine-tuned model weights for a particular task. Applying task vectors to pre-trained model weights via addition---and removing them via subtraction---is an intuitive way to alter model behavior and enhance or detract from performance on specific tasks. \\
\cmidrule{3-5}
  & 
  & \multirow{3}{\subwidth}{Model Breadcrumbs}
  & \citet{davari2023model} 
  & Takes task vectors from several fine-tuned models and limits destructive interference between task-specific parameters by masking outlier directions in each task vector. Suitable for applying Task Arithmetic~\cite{ilharco2022editing} to enhance performance in multiple tasks simultaneously. \\
\cmidrule{3-5}
  & 
  & \multirow{3}{\subwidth}{TIES-merging} 
  & \citet{yadav2024ties} 
  & Improves the performance and stability of Task Arithmetic~\cite{ilharco2022editing} when using multiple task vectors by identifying redundancies between task vectors, resolving sign conflicts between corresponding parameters in task vectors, and exclusively merging parameters that align with the final agreed-upon sign. \\
\cmidrule{3-5}
  & 
  & DARE
  & \citet{yu2024language} 
  & Builds upon Task Arithmetic~\cite{ilharco2022editing} by sparsifying task vectors, greatly reducing interference between merged parameters. DARE demonstrates that, in some cases, up to 90-99\% of fine-tuning parameters can be eliminated while preserving fine-tuning performance. This, in turn, can be exploited to efficiently create multi-task LLMs using model merging. \\
\cmidrule{2-5}
& \multirow{20}{\subwidth}{Data-Aware} 
  & FedAvg
  & \citet{sun2022decentralized} 
  & Computes a weighted average between source model parameters in a federated setting. Weights each source model's parameters by the proportion of the data in the federated system that is present at their node. Suitable for merging models whose data distributions are heterogeneous and non-IID. \\
\cmidrule{3-5}
  & 
  & AdaMerging
  & \citet{yang2023adamerging} 
  & Builds upon Task Arithmetic~\cite{ilharco2022editing}. Learns merging coefficients for task vectors adaptively by minimizing prediction entropy over unlabeled test data. Demonstrates strong multi-task performance, comparable with that of an ensemble. \\
\cmidrule{3-5}
  & 
  & \multirow{3}{\subwidth}{RegMean}
  & \citet{jin2022dataless} 
  & Merges weights at each layer by computing the least-squares fit to their activation maps. This ensures that the merged weight matrix produces activations similar to that of each source matrix when presented with data from that source model's training distribution.  \\
\cmidrule{3-5}
  & 
  & \multirow{4}{\subwidth}{ZipIt!}
  & \citet{stoica2023zipit} 
  & Identifies redundant parameters between models whose activations are highly correlated. This technique only merges redundant model parameters and preserves task-specific ones to prevent destructive interference when merging models. Demonstrates strong multi-task performance, even when models are trained independently.  \\
\cmidrule{3-5}
  & 
  & \multirow{3}{\subwidth}{Evolutionary Model Merging}
  & \citet{akiba2024evolutionary} 
  & Employs an evolutionary algorithm to learn whether to compose layers in sequence or merge them with a learned weighting. The final layer composition and weights for model merging are optimized to maximize training accuracy. \\
\cmidrule{2-5}
& \multirow{8}{\subwidth}{Information Theoretic} 
  & Fisher Weighted Averaging
  & \citet{matena2022merging} 
  & Computes a weighted average between source model parameters, with weights for each parameter defined by the Fisher information of that parameter. Applies a diagonal approximation of the Fisher Information matrix for computational tractability. \\
\cmidrule{3-5}
  & 
  & Merging by Matching Models in Task Parameter Subspaces (MaTS)
  & \citet{tam2023merging} 
  & Poses model merging as equivalent to solving a linear system of equations for the optimal merged parameter values. They design an enhanced Fisher Weighted Averaging procedure by using the Kronecker Factorization to obtain a more accurate block-diagonal approximation to the Fisher Information matrix. Computing the closed-form solution to this system is intractable in practice; therefore, they apply the method of Conjugate Gradients to find an approximate solution.  \\
\midrule
\multirow{29}{\subwidth}{Neuron Alignment}
& \multirow{15}{\subwidth}{Hard Alignment}  
  & Weight Matching 
  & \citet{ainsworth2022git}
  & Aligns corresponding layers of neurons between models of the same architecture by maximizing the similarity between their weight matrices (i.e., maximizing the Frobenius inner product of both weight matrices). They pose this problem as an NP-hard SOBLAP assignment problem and approximate a greedy solution using coordinate descent. Once weights are aligned, they are simply averaged. \\
\cmidrule{3-5}
  & 
  & Optimizing Mode Connectivity via Neuron Alignment
  & \citet{tatro2020optimizing} 
  & Presents a heuristic, ``neuron alignment'', which measures similarity between the distribution of activations between two weight matrices. They relate finding a permutation matrix which optimizes this metric to the assignment problem~\cite{burkard1999linear} and optimal transport. Weights are interpolated between once aligned.  \\
\cmidrule{3-5}
  & 
  & Probabilistic Federated Neural Matching (PFNM)
  & \citet{yurochkin2019bayesian} 
  & Aligns the parameters of edge models to a global model in a federated setting by using a non-parametric Bayesian model to determine the optimal assignment of neurons to one another for alignment and merging into a global model.  \\
\cmidrule{3-5}
  & 
  & Federated Learning with Matched Averaging (FedMA)
  & \citet{wang2020federated} 
  & Poses neuron alignment as an extended bipartite matching problem and applies the iterative Hungarian matching algorithm to solve the corresponding assignment problem, aligning neurons before merging.  \\
\cmidrule{2-5}
& \multirow{8}{\subwidth}{Soft Alignment}  
  & Optimal Transport Fusion (OTFusion) 
  & \citet{singh2020model}
  & Generalizes prior approaches which pose neuron alignment as a discrete assignment problem by modeling neuron alignment using the optimal transport framework. Use established techniques to solve the optimal transport problem to produce \enquote{soft} alignment maps between neurons, which can be used to align and combine corresponding layers between source models. \\
\cmidrule{3-5}
  & 
  & Transformer Fusion with Optimal Transport
  & \citet{imfeld2023transformer} 
  & Extends OTFusion~\cite{singh2020model} to handle modern Transformer architectures, also proposes a technique to align and merge models of heterogeneous architectures.  \\
\bottomrule
\end{tabular}
% \end{tabularx}
\end{adjustbox}
\end{table}

==> sections/old_survey_table.tex <==

\begin{longtable}{|P{0.12\textwidth}|p{0.1\textwidth}|P{0.1\textwidth}|P{0.09\textwidth}|p{0.59\textwidth}|}
\hline
Classification & Type & Name & Source & Summary \\
\hline
Weight Aggregation
  & \multirow{5}{\subwidth}{Weight Averaging} 
  & FedSGD (Simple Average)
  & \citet{mcmahan2017communication} 
  & Computes a simple average over source model parameters. Requires models of the same architecture. \\
\cline{3-5}
  & 
  & Stochastic Weighted Averaging 
  & \citet{izmailov2018averaging} 
  & Gathers checkpoints from various points in the training trajectory of a single model and computes a simple average over their parameters. \\
\cline{3-5}
  & 
  & Model Soup 
  & \citet{wortsman2022model} 
  & Takes the simple average of parameters from models of the same architecture fine-tuned with different hyperparameters. \\
\cline{3-5}
  & 
  & Sparse Soup 
  & \citet{zimmer2023sparse} 
  & Constructs model soups that are more efficient for inference by applying a technique inspired by Iterative Magnitude Pruning~\cite{tanaka2020pruning} to produce sparse models. \\
\cline{3-5}
  & 
  & SWAMP 
  & \citet{choi2023swamp} 
  & Iteratively applies Iterative Magnitude Pruning~\cite{tanaka2020pruning} and simple weight averaging between multiple fine-tuned models to produce a final sparse, merged model. \\
\cline{2-5}
& \multirow{4}{\subwidth}{Weight Steering} 
  & Task Arithmetic
  & \citet{ilharco2022editing} 
  & Computes a \enquote{task vector}: the difference between the pre-trained and fine-tuned model weights for a particular task. Applying task vectors to pre-trained model weights via addition---and removing them via subtraction---is an intuitive way to alter model behavior and enhance or detract from performance on specific tasks. \\
\cline{3-5}
  & 
  & Model Breadcrumbs 
  & \citet{davari2023model} 
  & Takes task vectors from several fine-tuned models and limits destructive interference between task-specific parameters by masking outlier directions in each task vector. Suitable for applying Task Arithmetic~\cite{ilharco2022editing} to enhance performance in multiple tasks simultaneously. \\
\cline{3-5}
  & 
  & TIES-merging 
  & \citet{yadav2024ties} 
  & Improves the performance and stability of Task Arithmetic~\cite{ilharco2022editing} when using multiple task vectors by identifying redundancies between task vectors, resolving sign conflicts between corresponding parameters in task vectors, and exclusively merging parameters that align with the final agreed-upon sign. \\
\cline{3-5}
  & 
  & DARE
  & \citet{yu2024language} 
  & Builds upon Task Arithmetic~\cite{ilharco2022editing} by sparsifying task vectors, greatly reducing interference between merged parameters. DARE demonstrates that, in some cases, up to 90-99\% of fine-tuning parameters can be eliminated while preserving fine-tuning performance. This, in turn, can be exploited to efficiently create multi-task LLMs using model merging. \\
\cline{2-5}
& \multirow{4}{\subwidth}{Data-Aware} 
  & FedAvg
  & \citet{sun2022decentralized} 
  & Computes a weighted average between source model parameters in a federated setting. Weights each source model's parameters by the proportion of the data in the federated system that is present at their node. Suitable for merging models whose data distributions are heterogeneous and non-IID. \\
\cline{3-5}
  & 
  & AdaMerging
  & \citet{yang2023adamerging} 
  & Builds upon Task Arithmetic~\cite{ilharco2022editing}. Learns merging coefficients for task vectors adaptively by minimizing prediction entropy over unlabeled test data. Demonstrates strong multi-task performance, comparable with that of an ensemble. \\
\cline{3-5}
  & 
  & RegMean
  & \citet{jin2022dataless} 
  & Merges weights at each layer by computing the least-squares fit to their activation maps. This ensures that the merged weight matrix produces activations similar to that of each source matrix when presented with data from that source model's training distribution.  \\
\cline{3-5}
  & 
  & ZipIt!
  & \citet{stoica2023zipit} 
  & Identifies redundant parameters between models whose activations are highly correlated. This technique only merges redundant model parameters and preserves task-specific ones to prevent destructive interference when merging models. Demonstrates strong multi-task performance, even when models are trained independently.  \\
\cline{2-5}
& \multirow{2}{\subwidth}{Information Theoretic} 
  & Fisher Weighted Averaging
  & \citet{matena2022merging} 
  & Computes a weighted average between source model parameters, with weights for each parameter defined by the Fisher information of that parameter. Applies a diagonal approximation of the Fisher Information matrix for computational tractability. \\
\cline{3-5}
  & 
  & Merging by Matching Models in Task Parameter Subspaces (MaTS)
  & \citet{tam2023merging} 
  & Poses model merging as equivalent to solving a linear system of equations for the optimal merged parameter values. They design an enhanced Fisher Weighted Averaging procedure by using the Kronecker Factorization to obtain a more accurate block-diagonal approximation to the Fisher Information matrix. Computing the closed-form solution to this system is intractable in practice; therefore, they apply the method of Conjugate Gradients to find an approximate solution.  \\
\hline
Neuron Alignment 
& \multirow{4}{\subwidth}{Hard Alignment}  
  & Weight Matching 
  & \citet{ainsworth2022git}
  & Aligns corresponding layers of neurons between models of the same architecture by maximizing the similarity between their weight matrices (i.e., maximizing the Frobenius inner product of both weight matrices). They pose this problem as an NP-hard SOBLAP assignment problem and approximate a greedy solution using coordinate descent. Once weights are aligned, they are simply averaged. \\
\cline{3-5}
  & 
  & Optimizing Mode Connectivity via Neuron Alignment
  & \citet{tatro2020optimizing} 
  & Presents a heuristic, \enquote{neuron alignment}, which measures similarity between the distribution of activations between two weight matrices. They relate finding a permutation matrix which optimizes this metric to the assignment problem~\cite{burkard1999linear} and optimal transport. Weights are interpolated between once aligned.  \\
\cline{3-5}
  & 
  & Probabilistic Federated Neural Matching (PFNM)
  & \citet{yurochkin2019bayesian} 
  & Aligns the parameters of edge models to a global model in a federated setting by using a non-parametric Bayesian model to determine the optimal assignment of neurons to one another for alignment and merging into a global model.  \\
\cline{3-5}
  & 
  & Federated Learning with Matched Averaging (FedMA)
  & \citet{wang2020federated} 
  & Poses neuron alignment as an extended bipartite matching problem and applies the iterative Hungarian matching algorithm to solve the corresponding assignment problem, aligning neurons before merging.  \\
\cline{2-5}
& \multirow{4}{\subwidth}{Soft Alignment}  
  & Optimal Transport Fusion (OTFusion) 
  & \citet{singh2020model}
  & Generalizes prior approaches which pose neuron alignment as a discrete assignment problem by modeling neuron alignment using the optimal transport framework. Use established techniques to solve the optimal transport problem to produce \enquote{soft} alignment maps between neurons, which can be used to align and combine corresponding layers between source models. \\
\cline{3-5}
  & 
  & Transformer Fusion with Optimal Transport
  & \citet{imfeld2023transformer} 
  & Extends OTFusion~\cite{singh2020model} to handle modern Transformer architectures, also proposes a technique to align and merge models of heterogeneous architectures.  \\
\hline
\caption{Table of Model Merging techniques covered in this work, categorized by their approach}
\end{longtable}





==> sections/problem.tex <==
...

==> sections/system.tex <==
...

==> sections/weight_averaging_table.tex <==
\begin{longtable}{|P{0.15\textwidth}|P{0.34\textwidth}|P{0.09\textwidth}|p{0.4\textwidth}|}
\hline
Classification & Name & Source & Summary \\
\hline
Weight Averaging
  & FedSGD (Simple Average)
  & \citet{mcmahan2017communication} 
  & Computes a simple average over source model parameters. Requires models of the same architecture. \\
\cline{2-4}
  & Stochastic Weighted Averaging 
  & \citet{izmailov2018averaging} 
  & Gathers checkpoints from various points in the training trajectory of a single model and computes a simple average over their parameters. \\
\cline{2-4}
  & Model Soup 
  & \citet{wortsman2022model} 
  & Takes the simple average of parameters from models of the same architecture fine-tuned with different hyperparameters. \\
\cline{2-4}
  & Sparse Soup 
  & \citet{zimmer2023sparse} 
  & Constructs model soups that are more efficient for inference by applying a technique inspired by Iterative Magnitude Pruning~\cite{tanaka2020pruning} to produce sparse models. \\
\cline{2-4}
  & SWAMP 
  & \citet{choi2023swamp} 
  & Iteratively applies Iterative Magnitude Pruning~\cite{tanaka2020pruning} and simple weight averaging between multiple fine-tuned models to produce a final sparse, merged model. \\
\hline
\end{longtable}


==> sections/weight_steering_table.tex <==
\begin{longtable}{|P{0.15\textwidth}|P{0.34\textwidth}|P{0.09\textwidth}|p{0.4\textwidth}|}
\hline
Classification & Name & Source & Summary \\
\hline
Weight Steering
  & Task Arithmetic
  & \citet{ilharco2022editing} 
  & Computes a \enquote{task vector}: the difference between the pre-trained and fine-tuned model weights for a particular task. Applying task vectors to pre-trained model weights via addition---and removing them via subtraction---is an intuitive way to alter model behavior and enhance or detract from performance on specific tasks. \\
\cline{2-4}
  & Model Breadcrumbs 
  & \citet{davari2023model} 
  & Takes task vectors from several fine-tuned models and limits destructive interference between task-specific parameters by masking outlier directions in each task vector. Suitable for applying Task Arithmetic~\cite{ilharco2022editing} to enhance performance in multiple tasks simultaneously. \\
\cline{2-4}
  & TIES-merging 
  & \citet{yadav2024ties} 
  & Improves the performance and stability of Task Arithmetic~\cite{ilharco2022editing} when using multiple task vectors by identifying redundancies between task vectors, resolving sign conflicts between corresponding parameters in task vectors, and exclusively merging parameters that align with the final agreed-upon sign. \\
\cline{2-4}
  & DARE
  & \citet{yu2024language} 
  & Builds upon Task Arithmetic~\cite{ilharco2022editing} by sparsifying task vectors, greatly reducing interference between merged parameters. DARE demonstrates that, in some cases, up to 90-99\% of fine-tuning parameters can be eliminated while preserving fine-tuning performance. This, in turn, can be exploited to efficiently create multi-task LLMs using model merging. \\
\hline
\end{longtable}

